Variance function estimation in high-dimensions

We consider the high-dimensional heteroscedastic regression model, where the mean and the log variance are modeled as a linear combination of input variables. Existing literature on high-dimensional linear regres- sion models has largely ignored non-constant error variances, even though they commonly occur in a variety of applications ranging from biostatis- tics to finance. In this paper we study a class of non-convex penalized pseudolikelihood estimators for both the mean and variance parameters. We show that the Heteroscedastic Iterative Penalized Pseudolikelihood Optimizer (HIPPO) achieves the oracle property, that is, we prove that the rates of convergence are the same as if the true model was known. We demonstrate numerical properties of the procedure on a simulation study and real world data.

==> table_zero_mean_exper2.tex <==
% This table was planned to be put in Example 2. However, it did not
% make the cut. It demonstrates the performance on estimating the
% variance parameter when the mean is known.
%


% \begin{table}[t]
% {
% \hfill{}
% \begin{tabular}{l@{\hspace{0.3cm}}ccc}
%   &  $\norm{\theta - \hat\theta}_2$  &
%      ${\sf Pre}_{\theta}$ & ${\sf Rec}_{\theta}$ \\
% \cline{2-4}
% \vspace{-0.2cm}
% \\
% &\multicolumn{3}{c}{\underline{$n = 200$}} \\
% \vspace{-0.2cm}
% \\
% HHR-AIC & 0.74(0.15) & 0.28(0.10) & 1.00(0.02) \\
% HIPPO-AIC  & 1.10(0.34) & 0.27(0.17) & 0.94(0.062) \\
% HHR-BIC & 0.77(0.15) & 0.55(0.11) & 0.99(0.03) \\
% HIPPO-BIC  & 1.10(0.30) & 0.58(0.17) & 0.89(0.09) \\
% \\
% &\multicolumn{3}{c}{\underline{$n = 400$}} \\
% \vspace{-0.2cm}
% \\
% HHR-AIC & 0.44(0.07) & 0.27(0.13) & 1.00(0.00) \\
% HIPPO-AIC & 0.43(0.12) & 0.48(0.23) & 1.00(0.02) \\
% HHR-BIC & 0.47(0.09) & 0.67(0.14) & 1.00(0.00) \\
% HIPPO-BIC  & 0.60(0.19) & 0.83(0.13) & 0.98(0.04) \\
% \hline
% \hline
% \end{tabular}
% }
% \hfill{}
% \caption{
%   Mean (sd) performance of HHR and \acro under the model in
%   Example~2 (averaged over 100 independent runs). The mean parameter
%   $\betab$ is assumed to be known.
% }
% \label{tb:zero_mean_exper2}
% \end{table}


